The phase curve and the geometric albedo of WASP-43b measured with CHEOPS, TESS and HST WFC3/UVIS

Observations of the phase curves and secondary eclipses of extrasolar planets provide a window on the composition and thermal structure of the planetary atmospheres. For example, the photometric observations of secondary eclipses lead to the measurement of the planetary geometric albedo $A_g$, which is an indicator of the presence of clouds in the atmosphere. In this work we aim to measure the $A_g$ in the optical domain of WASP-43b, a moderately irradiated giant planet with an equilibrium temperature of $\sim$1400~K. To this purpose, we analyze the secondary eclipse light curves collected by CHEOPS, together with TESS observations of the system and the publicly available photometry obtained with HST WFC3/UVIS. We also analyze the archival infrared observations of the eclipses and retrieve the thermal emission spectrum of the planet. By extrapolating the thermal spectrum to the optical bands, we correct the optical eclipses for thermal emission and derive the optical $A_g$. The fit of the optical data leads to a marginal detection of the phase curve signal, characterized by an amplitude of $160\pm60$~ppm and 80$^{+60}_{-50}$~ppm in the CHEOPS and TESS passband respectively, with an eastward phase shift of $\sim50^\circ$ (1.5$\sigma$ detection). The analysis of the infrared data suggests a non-inverted thermal profile and solar-like metallicity. The combination of optical and infrared analysis allows us to derive an upper limit for the optical albedo of $A_g<0.087$ with a confidence of 99.9\%. Our analysis of the atmosphere of WASP-43b places this planet in the sample of irradiated hot Jupiters, with monotonic temperature-pressure profile and no indication of condensation of reflective clouds on the planetary dayside.

==> previous.tex <==
\section{Previous works {\bf TO BE REMOVED IN THE FINAL VERSION}}

Copy-paste of previous papers, just to collect all the info in one place.

\subsection{\citet{Hellier2011}} The 2009 WASP-South data show a modulation at a period of 15.6 ± 0.4 d with a significance of >99.9\% (Fig. 2), plus its first harmonic at 7.8 d. The amplitude is 0.006 ± 0.001 mag. The 2010 data (not shown) show the same modulation less clearly, but still with a significance of >99\%. Most likely 15.6 d is the rotational period of WASP-43. If Prot were instead at the 7.8-d period then the dominant power would be at twice Prot , which is unfeasible for any spot pattern.

Taking the rotation period as 15.6 d, and with the radius from Table 2, gives an equatorial velocity of v = 2.0 +- 0.1 km s-1 . This is significantly lower than the measured v sin I, which suggests that there is additional broadening in the lines. For example the two are reconciled by increasing macroturbulence to 3 km s-1 . The 15.6-d rotation rate implies a gyrochronological age of 400+200-100  Myr, using the Barnes (2007) relation. However, this would assume that the star has not been spun up by tidal interactions with the planet; an alternative possibility is that the star could be significantly older, but has been spun up by tidal interactions that will eventually destroy the planet (see, e.g., Brown et al. 2011).

\subsection{\citet{Gillon2012}}

{\bf We detected the emission of the planet at 2.09 um (lambda = 2.095 um, width = 0.020 um) at better than 11$\sigma$, the deduced occultation depth being 1560 +- 140 ppm. Our detection of the occultation at 1.19 um (lambda = 1.186 um,
width = 0.020 um) is marginal (790 +- 320 ppm) and more observations would be needed to confirm it. We place a 3$\sigma$ upper limit of 850 ppm on the depth of the occultation at $\sim$0.9 um (lambda = 915.9 +- 0.5 nm).} Together, these results strongly favor a poor redistribution of the heat from the dayside to the nightside of the planet, and marginally favor a model with no day-side temperature inversion.

\subsection{Wang 2013}

We report new detections of thermal emission from the transiting hot Jupiter WASP-43b in the H and Ks bands as observed at secondary eclipses. The observations were made with the WIRCam instrument on the Canada-France–Hawaii Telescope. {\bf We obtained a secondary eclipse depth of 0.103+0.017-0.017\% and 0.194-0.029+0.029\% in the H and Ks bands, respectively.}

Our observations constrain the thermal structure of the lower atmosphere of WASP-43b. Since the photometric H and Ks bands are relatively devoid of strong molecular absorption compared to the Spitzer IRAC bands (see, e.g., Madhusudhan et al. 2011a), observations in these bands probe the deepest layers in the atmosphere from where emergent flux travels relatively unimpeded to the observer. For highly irradiated giant planets, the temperature profile in the optically thick regime of the dayside atmosphere is expected to be isothermal (Hansen 2008; Guillot 2010). As such, the brightness temperatures observed in the H and Ks bands constrain the isothermal temperature structure at the $\tau\sim1$ surface, or the planetary “photosphere,” of the dayside atmosphere of WASP-43b. Our observed planet-star flux ratios in the H and Ks bands are shown in Figure 6, together with the narrow-band photometric data reported by Gillon et al. (2012) at 1.19 um and 2.095 um. We find that the sum-total of available data can be explained by a blackbody spectrum of the planet with a temperature of 1850 K, representing the isotherm in the lower atmosphere.

Assuming a solar abundance composition, we find that models fitting the data require very low day–night energy redistribution ($\lesssim15\%$), consistent with the finding of Gillon et al. (2012).

Our data are unable to rule out the presence of a weak temperature inversion: one with only a marginal temperature excess ($\lesssim$100 K) over the isotherm of the lower atmosphere or one where the inversion occurs in regions of low molecular opacity, e.g., for pressures below $\sim$10-2 bar. A thermal inversion in WASP-43b is also less likely on theoretical grounds if molecules such as TiO and VO are the cause of thermal inversions in hot Jupiters (Hubeny et al. 2003; Fortney et al. 2008). We find that the best fitting temperatures of the lower atmosphere as constrained by our data are cooler than the condensation curve of TiO at the same pressures, which would lead to the formation of a TiO cold trap. The TiO/VO condensation together with their gravitational settling, owing to their large molecular mass, would make it unlikely for gaseous TiO/VO to remain aloft in the atmosphere in the significant amounts required to cause thermal inversions (Spiegel et al. 2009).

\subsection{Chen 2014}

We observed one transit and one occultation event simultaneously in the g', r', i', z', J, H, K bands using the GROND instrument on the MPG/ESO 2.2-m telescope.

We performed a tentative analysis on the wavelength dependent transit depths. No significant variation in transit depths was found, with the largest deviation of 1.6$\sigma$, 1.5$\sigma$, and 1.6$\sigma$ in the i', H, and K-bands, respectively. Our broad-band transmission spectrum can be explained by either (i) a flat featureless straight line that indicates thick clouds; (ii) atomic Na/K, or molecular TiO/VO imprinted spectra that indicate a cloud-free atmosphere; or (iii) a Rayleigh scattering profile that indicates high-altitude hazes. 

{\bf We detected a flux ratio during occultation of 0.197+-0.042\% in the GROND K-band and 0.037+0.023-0.021\% in the GROND i-band (Fig.~\ref{tab:chen}).} Before comparing them to theoretical models, we first estimated their brightness temperatures. The planetary dayside thermal emission was simplified as a blackbody, while the stellar flux was interpolated from the Kurucz stellar models (Kurucz 1979) with the values of T eff , log g, and [Fe/H] derived from this work. The K-band occultation detection is translated into a brightness temperature of 1878+108-116 K, while the i-band detection corresponds 2225+139-225 K. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Chen_table.pdf}
    \caption{From Chen+2014}
    \label{tab:chen}
\end{figure}

We confirm that the dayside atmosphere is very inefficient for heat redistribution. We tentatively detected the dayside flux of WASP-43b in the i'-band with a flux ratio of 0.037 +0.023-0.021\%. Its brightness temperature 2225 K is too high to be explained solely by the assumption of an isothermal blackbody. We performed tentative analysis involving the Rayleigh scattering caused by reflective hazes present in the upper atmosphere of the dayside. A firm conclusion cannot be drawn based on current optical measurements.


\subsection{Blecic 2014}

{\bf The eclipse depths and brightness temperatures from our jointly fit model are 0.347\% +- 0.013\% and 1670 +- 23 K at 3.6 um and 0.382\% ± 0.015\% and 1514 +- 25 K at 4.5 um.}


We constrain the thermal structure and composition of WASP-43b by combining our Spitzer photometric observations at 3.6 um and 4.5 um combined with previously reported ground-based narrow-band photometric data from Gillon et al. (2012), obtained using VLT/HAWK-I at 1.19 um and 2.09 um, and broadband photometric data from Wang et al. (2013) obtained using CFHT/WIRCAM in the H (1.6 um) and Ks (2.1 um) bands. The data also place a joint constraint on the day–night energy redistribution and the Bond albedo by requiring global energy balance, i.e., that the integrated emergent power from the planet does not exceed the incident irradiation. Given that
the number of model parameters is >=10 (depending on the C/O ratio) and the number of available data points is 6, our goal is to
find the regions of model space favored by the data, rather than to determine a unique fit. We explore the model parameter space
by using an MCMC routine (for details, see Madhusudhan \& Seager 2009, 2010; Madhusudhan et al. 2011a).

The data rule out a strong thermal inversion in the dayside atmosphere of WASP-43b. The data and two model spectra of atmospheres without thermal inversions are shown in Figure 8. The ground-based and Spitzer data provide complementary constraints on the atmospheric properties. The ground-based photometric bandpasses, in narrow bands at 1.19 um and 2.09 um (Gillon et al. 2012) and in broad bands at 1.6 um and 2.1 um (Wang et al. 2013), span spectral regions of low molecular opacity and hence probe the deep layers of the atmosphere at pressures of P $\sim$ 1 bar, beyond which the atmosphere is optically thick because of collision-induced opacity (the contribution functions are given in Figure 9). Consequently, the brightness temperatures from such ground-based data constrain the isothermal temperature structure of the deep atmosphere (Madhusudhan 2012). On the other hand, the two Spitzer data
sets show lower brightness temperatures at 3.6 um and 4.5 um relative to the ground-based data, which is possible only if
the temperature structure is decreasing outward in the atmosphere, causing molecular absorption in the Spitzer bands. The presence of a strong thermal inversion, on the contrary, would have caused molecular emission leading to higher brightness temperatures in the Spitzer bands relative to the ground-based bands. Consequently, the sum total of Spitzer and ground-based data rule out a strong thermal inversion in WASP-43b’s dayside photosphere.

Our population of model fits to the combined Spitzer and ground-based data allow for up to $\sim$35\% day–night energy redistribution in the planet. Among the acceptable models, those with higher $f_r$ values require cooler lower atmospheres on the dayside and hence predict lower fluxes in the ground-based channels. 

The lack of a strong thermal inversion in WASP-43b is not surprising. At an equilibrium temperature of $\sim$1400 K, the dayside atmosphere of WASP-43b is not expected to host gaseous TiO and VO, which have been proposed to cause thermal inversions (Spiegel et al. 2009; Hubeny et al. 2003; Fortney et al. 2008), though hitherto unknown molecules that could also potentially cause such inversions cannot be ruled out (Zahnle et al. 2009). The lack of a thermal inversion is also consistent with the hypothesis of Knutson et al. (2010), since the host star WASP-43 is known to be active (Hellier et al. 2011).

\subsection{Kreidberg 2014}

We observed three full-orbit phase curves, three primary transits, and two secondary eclipses of WASP-43b with 61 HST orbits as part of GO Program 13467. During the observations, we obtained low-resolution time series spectroscopy with the WFC3 G141 grism over the wavelength range 1.1–1.7 um. In our analysis, we used a subset of the total observations, including only spectra obtained within 160 minutes of the time of central transit or eclipse.

{\bf The eclipse depths are in Fig.~\ref{tab:kreidberg}.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Kreidberg_table.pdf}
    \caption{From Kreidberg+2014}
    \label{tab:kreidberg}
\end{figure}

The emission spectrum shows strong evidence for water absorption. We detect water at 11.7$\sigma$ confidence (6.4$\sigma$ from the WFC3 data alone). Water is the only molecule significantly detected over the WFC3 wavelength range; however, additional constraints from the Spitzer data suggest CO and/or CO2 are also present in the planet’s atmosphere. We detect CO+CO2 at 4.7$\sigma$ confidence in the combined WFC3/IRAC spectrum.  

The transmission spectrum fit allows a water volume mixing ratio between 3.3$\times$10-5 and 1.4$\times$10-3 at 1$\sigma$, which is consistent with the bounds derived from the emission measurements. No other molecules are detected in the spectrum according to the BIC.

\subsection{Stevenson 2014}

All of the observations used the HST WFC3/G141 grism (1.1 to 1.7 um). We produced time-series spectroscopy by dividing the spectra into 15 0.035-mm-wide channels (7 pixels, resolution R = l/Dl $\sim$ 37). We also produced band-integrated “white” light curves to resolve finer details in the shape of the phase curve (Fig. 1).

The flux peaks prior to secondary eclipse (eastward of the substellar point) and then decreases until the planet transits in front of its host star. Because the phase curve minimum occurs west of the antistellar point, we detect a strong asymmetry ($\sim$10s) in the shape of the observed phase curve. We measure a white light curve eclipse depth that is consistent with the peak-to-peak planet flux variation. This confirms a relatively cool night side and poor heat redistribution. 

{\bf We gain additional information by decomposing the white light phase curve into 15 spectrophotometric channels (Fig.~\ref{tab:stevenson}).} The spectrally resolved phase curves exhibit wavelength-dependent amplitudes, phase shifts, and eclipse depths (table S2).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Stevenson_table.pdf}
    \caption{From Stevenson+2014}
    \label{tab:stevenson}
\end{figure}



We find that water is the only absorber to significantly influence the phase-resolved emission spectra we find that the planet redistributes heat poorly [(19), heat redistribution factor F 0.503+0.021-0.003 , where F 0.5-1 spans the range from zero to full heat redistribution].

We find a Bond albedo of 0.18+0.07-0.12.

The retrieved thermal profiles are consistent with a global, monotonically decreasing temperature with altitude, as would be expected from radiative cooling without high-altitude absorbers of stellar radiation.

Phase-curve peaks prior to the time of secondary eclipse (as seen in Fig. 1) have previously been reported in hot Jupiters (1, 6) and match predictions from three-dimensional (3D) circulation models (30–32). Such models show that the eastward offset results from a strong jet stream at the equator; our observations thus suggest that WASP-43b exhibits such an eastward-flowing jet. 

\subsection{Stevenson 2017}

Using the Spitzer Space Telescope, we obtained a total of three phase curve observations of WASP-43b (P=0.813 days) at 3.6 and 4.5 um.

We detect a strong asymmetry in the 4.5 um phase curve that is similar in shape to the HST/WFC3 band-integrated phase curve (Stevenson et al. 2014, see Figure 2). The median phase curve maximum is shifted by 21.1+-1.8 degrees east of the substellar point. The median phase curve minimum occurs 6.8+-2.7 degrees west of the anti-stellar point. Therefore, the maximum planetary emission occurs 0.421+-0.009 orbits after the observed minimum, which is consistent at the 1.5$\sigma$ level with our reported WFC3 difference (0.436+-0.005 orbits, Stevenson et al. 2014). This suggests that these two wavelength regions probe similar depths within WASP-43b’s atmosphere.

{\bf In addition to the phase curves offset, we measure a peak-to-peak amplitude, Ap2p, of 0.399+-0.014\% at 4.5 um. Note that since the maximum flux occurs prior to secondary eclipse, it is physically plausible for Ap2p to exceed the secondary eclipse depth (0.383+-0.008\%).}

When fit individually the two 3.6 um phase curves, we determine that the second visit more accurately reflects WASP-43b’s typical
nightside emission and, thus, adopt those data for further analysis and interpretation. For the second 3.6 um visit, the median phase curve maximum and minimum are shifted by 12.2+-1.7 degrees East and 9+-5 degrees West of the substellar and anti-stellar points. The maximum-to-minimum orbital phase difference of 0.442+-0.016 is consistent with both the WFC3 and 4.5 um values. {\bf The eclipse depth at 3.6 um is 0.323+-0.006\%.}

{\bf The summary of the HST depths (from Kreidberg2014) and Spitzer depths (from Stevenson2017) is in Fig.~\ref{tab:stevenson2017}.}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Stevenson2017_table.pdf}
    \caption{From Stevenson+2017}
    \label{tab:stevenson2017}
\end{figure*}

The slope in the transmission spectrum (DZ J-LM/H=5.1+-1.1) suggests the presence of hazes that are partially obscuring the signal (Sing et al. 2016). This is consistent with the need for a cloud deck in our WFC3 atmospheric retrieval (Kreidberg et al. 2014) and the interpretation of Stevenson (2016), in which we find that the WFC3 water feature only extends 1.1+-0.5 planetary scale heights. A cloud-free atmosphere should exhibit spectral features that extend over several scale heights.

Using transit times that span more than four years, we find no significant evidence for tidal decay in the orbit of WASP-43b.

Interestingly, the cloud-free GCM phase curves by Kataria et al. (2015) fit the data from the first 3.6 um visit at most orbital phases. Therefore, the strong nightside emission could be explained by a temporary hole in a hypothesized nightside cloud deck. Repeated phase curve observations would be necessary to search for additional signs of variability before any conclusions could be drawn. Until then, the source of the nightside flux inconsistency remains a mystery. For the remainder of this investigation, we adopt the phase curve data from the second 3.6 um visit.

We derive a precise metallicity constraint of 0.4-1.7$\times$ solar at 1$\sigma$ confidence. This value is consistent with our previous estimate (0.4–3.5$\times$, Kreidberg et al. 2014) based on the WFC3+IRAC transit and eclipse data alone. The retrieved CO+CO2 abundance is constant with orbital phase. We estimate a global log abundance of -3.5+-0.4 and a nearly identical metallicity constraint of 0.3–1.7$\times$ solar. 

When we compare the Spitzer data to GCM phase curves, we achieve good fits on the planet dayside; however, the models over-predict emission on the planet nightside. This discrepancy could be explained by the presence of optically thick clouds, which are not included in the GCMs. However, one must then explain why other observed exoplanets with similar brightness temperatures more closely match their predicted nightside emission levels without the need for obscuring clouds (Knutson et al. 2012; Zellem et al. 2014).

\subsection{Mendon\c{c}a 2018}

{\bf In comparing both 3.6 um phase curves, we find amplitudes of 2395+-190 and 2719+-200 ppm for the two 3.6 um phase curves, compared to the previously published 2440+-230 and 3380+-110 ppm values. We also perform an analysis of the Spitzer 4.5 um data with the same photometric baseline model for which we find a phase-curve amplitude of 3258+-250 ppm.}

Confronting our GCM predictions with data leads us to conclude that clouds on the nightside of WASP-43b are necessary, and that constraints on the cloud-top pressure and longitudinal position of the cloud deck are obtained. There is a hint that enhanced CO2 abundances are present at and near the nightside of WASP-43b.

\subsection{Fraine 2021}

We photometrically observed the hot Jupiter system WASP-43 during an eclipse event of the planet. Our program was one of the first transiting exoplanet programs to use HST WFC3/UVIS (F350LP filter; 346–822 nm) in photometric scanning mode.

The overarching result from our observations is that the dayside of WASP-43b is very dark. Integrated over the entire optical band (346–822 nm), {\bf we derived an upper limit to the reflected light eclipse depth of less than 67 ppm, corresponding to a geometric albedo of Ag $\lesssim$ 0.06 (3$\sigma$ upper limit).} Our lack of detection of an optical eclipse depth implies a lack of reflective clouds on the dayside within the layers probed by eclipse observations (P$\lesssim$1 bar).

We explored the possible atmospheric scenarios using pressure–temperature files and the associated vertical mixing profiles (Kzz) generated in the GCMs from Kataria et al. (2014), which assume a cloudless atmosphere in chemical equilibrium. We used the cloud code developed by Ackerman \& Marley (2001) to compute cloud profiles derived from temperature–pressure profiles from Kataria et al. (2014). We allow Na2S, MnS, Cr, and MgSiO3 to condense. We also test five sedimentation efficiencies, fsed, which control the particle size and vertical extent of the cloud. A smaller fsed yields clouds that are vertically extensive, while larger fsed values yield vertically thin clouds. We then used PICASO (Batalha et al. 2019) to generate the geometric albedo spectrum of each case (36 cases), i.e., when the full-phase dayside appears at secondary eclipse.

Our modeling results (described in Section 4) revealed that to sustain this nondetected reflected light eclipse, the dayside atmosphere must significantly lack particles lofted into the observable part of the atmosphere. The models suggest that only the most lofted cloud case scenario, fsed = 0.1, could escape a cold trap at the deepest layers of the atmosphere to condense into a second upper cloud layer, which could lead to a detectable optical eclipse depth. All of the rest of our modeled sedimentation efficiencies led to particles being trapped at deeper pressures; they were thus unable to be mixed upward and recondensed. The fact that we did not detect an optical eclipse confirms that we can rule out a high-altitude, bright, uniform cloud layer.

